Adversarial Multi-Source Transfer Learning in Healthcare: Application to Glucose Prediction for Diabetic People

Deep learning has yet to revolutionize general practices in healthcare, despite promising results for some specific tasks. This is partly due to data being in insufficient quantities hurting the training of the models. To address this issue, data from multiple health actors or patients could be combined by capitalizing on their heterogeneity through the use of transfer learning. To improve the quality of the transfer between multiple sources of data, we propose a multi-source adversarial transfer learning framework that enables the learning of a feature representation that is similar across the sources, and thus more general and more easily transferable. We apply this idea to glucose forecasting for diabetic people using a fully convolutional neural network. The evaluation is done by exploring various transfer scenarios with three datasets characterized by their high inter and intra variability. While transferring knowledge is beneficial in general, we show that the statistical and clinical accuracies can be further improved by using of the adversarial training methodology, surpassing the current state-of-the-art results. In particular, it shines when using data from different datasets, or when there is too little data in an intra-dataset situation. To understand the behavior of the models, we analyze the learnt feature representations and propose a new metric in this regard. Contrary to a standard transfer, the adversarial transfer does not discriminate the patients and datasets, helping the learning of a more general feature representation. The adversarial training framework improves the learning of a general feature representation in a multi-source environment, enhancing the knowledge transfer to an unseen target. The proposed method can help improve the efficiency of data shared by different health actors in the training of deep models.

==> algorithms/dpr.tex <==
\RestyleAlgo{ruled}
\LinesNumbered

\begin{algorithm}
 \KwData{features F and domain D of S samples}
%  \KwResult{Domain Proximity Ratio (DPR)}
 \KwResult{Domains Relative Distance (DRD)}
 
 \For{$i=1 \rightarrow S$}{
 $F_i \leftarrow$ features of sample i\;
 $D_i \leftarrow$ class of sample i\;
%  $dist_i \leftarrow  \min_{F_j,j\in[1..S], j\neq i}{||F_i - F_j||^2}$\;
%  $dist_i^* \leftarrow  \min_{j\in[1..S], j\neq i, D_j \neq D_i}{||F_i - F_j||^2}$\;
$dist_i \leftarrow  ||F - F_i||^2$\;
$dist_i^* \leftarrow  dist_i[D \neq D_i]$\;

$mindist_i \leftarrow min(dist_i[1..i-1,i+1,..S]) $\;
$mindist_i^* \leftarrow min(dist_i^*)$\;

 $DRD_i  \leftarrow mindist_i^* / mindist_i$\;
 }
 
 $DRD \leftarrow 1/S \cdot \sum_{i=1}^{S}{DRD_i}$ \;
 \KwRet{DRD}\;
 \caption{Computation of the DRD metric}
 \label{algo:OCPR}
\end{algorithm}

==> tables/features_metrics.tex <==

% \newcolumntype{C}{>{\centering\arraybackslash}X}
% \newcolumntype{Z}[1]{>{\centering}m{#1}}


\begin{table}
    \caption{Measure of the ability of the pre-transfer models to compute general features, expressed in two different metrics: the domains relative distance (DRD) and the domain-neighbourhood perplexity (DNP). The mean (standard deviation) of the metrics are computed in the IOT$\rightarrow$O transfer scenario, averaging on the cross-validation folds and on the target subjects.}
    \label{table:features_res}
    \begin{tabularx}{\linewidth}{c|c||C|C|C|C}
            \toprule
            
            \multicolumn{2}{c||}{\textbf{Datasets}} & \multicolumn{2}{c|}{\textbf{DRD}} & \multicolumn{2}{c}{\textbf{DNP}} \\
            
            \midrule
            
            \textbf{S} & \textbf{T} & \textbf{TL} & \textbf{ATL} & \textbf{TL} & \textbf{ATL} \\
            
            \midrule
            % \scriptsize{()} &  \scriptsize{()} &  \scriptsize{()} &  \scriptsize{()}
            % \multicolumn{6}{c}{\textit{Measured on t-SNE features}} \\
            % \midrule
            % % I & \textcolor{cyan}{I} & &  0.60 & &  0.83 \\
            % I & O & 5.37 & \textcolor{cyan}{0.60} & 1.79 & \textcolor{cyan}{0.83} \\
            % O & O  &  4.18 & 0.67 & 1.61 & 0.83 \\
            % T & O  & 4.68 & 0.57 & 3.18 & 0.65 \\
            % IO & O  & 3.24 & 0.48 & 1.57 & 0.66 \\
            % IOT & O  & 3.88 & 0.26 & 2.55 & 0.35 \\
            
            % \midrule
            % \multicolumn{6}{c}{\textit{Measured on raw features}} \\
            % \midrule
            
            % I & \textcolor{cyan}{I} & & & 0.66 & & & 0.79 \\
            % I & O  & 1.39 & 0.61  & 1.07 & 0.75 \\
            % O & O  & 1.20 & 0.71  & 1.03 & 0.75\\
            % T & O  & 1.42 & 0.58  & 1.27 & 0.68\\
            % IO & O  & & 0.50  & 1.05 & 0.57 \\
            % IOT & O  & & 0.29  & & 0.35\\
            
            
            
            I & O  & 4.42 \scriptsize{(1.77)} & \textbf{2.34 \scriptsize{(1.38)}} & 0.61 \scriptsize{(0.04)} & \textbf{0.75 \scriptsize{(0.04)}} \\
            O & O  & 1.64 \scriptsize{(0.10)} & \textbf{1.11 \scriptsize{(0.03)}}  & 0.71 \scriptsize{(0.04)} & \textbf{0.74 \scriptsize{(0.03)}} \\
            T & O  & 18.21 \scriptsize{(5.01)} & \textbf{7.03 \scriptsize{(2.75)}}  & 0.58 \scriptsize{(0.02} & \textbf{0.68 \scriptsize{(0.02)}} \\
            IO & O  & 2.22 \scriptsize{(0.68)} & \textbf{1.46 \scriptsize{(0.29)}}  & 0.50 \scriptsize{(0.04)} & \textbf{0.57 \scriptsize{(0.02)}} \\
            IOT & O  & 6.78 \scriptsize{(1.65)} & \textbf{3.72 \scriptsize{(1.02)}}  & 0.29 \scriptsize{(0.01)} & \textbf{0.34 \scriptsize{(0.01)}} \\
            
            % I  & \multirow{7}{*}{I} & 16.46 \scriptsize{(4.24)} & 8.07 \scriptsize{(1.01)} & 15.42 \scriptsize{(3.97)} & 7.43 \scriptsize{(0.84)} \\
            % O &  & 16.35 \scriptsize{(4.22)} & 8.02 \scriptsize{(1.00)} & 15.82 \scriptsize{(3.97)} &  7.74 \scriptsize{(0.90)} \\
            % T &  & 17.97 \scriptsize{(4.74)} & 8.80 \scriptsize{(1.22)} & 17.88 \scriptsize{(4.85)} & 8.54 \scriptsize{(1.02)} \\
            % IO &  & \textit{15.71 \scriptsize{(4.12)}} & \textit{7.70 \scriptsize{(0.97)}} & 15.30 \scriptsize{(3.78)} & 7.43 \scriptsize{(0.78)} \\
            % IT &  & 16.24 \scriptsize{(4.23)} &  8.02 \scriptsize{(0.94)} & 15.39 \scriptsize{(4.05)} & 7.42 \scriptsize{(0.82)} \\
            % OT &  & 16.21 \scriptsize{(4.18)} & 7.94 \scriptsize{(1.01)} & 15.64 \scriptsize{(4.09)} & 7.49 \scriptsize{(0.83)} \\
            % IOT &  & 15.75 \scriptsize{(4.18)} & 7.75 \scriptsize{(1.00)} & \textbf{15.23 \scriptsize{(3.87)}} & \textbf{7.32 \scriptsize{(0.74)}} \\
            
            % \midrule
            
            % I  & \multirow{7}{*}{O} & 20.85 \scriptsize{(2.72)} & 10.34 \scriptsize{(1.79)} &  20.55 \scriptsize{(2.68)} & 10.08 \scriptsize{(1.71)} \\
            % O & & 20.79 \scriptsize{(2.70)} & 10.22 \scriptsize{(1.70)} & 20.56 \scriptsize{(2.55)} & 10.08 \scriptsize{(1.60)} \\
            % T &  & 22.65 \scriptsize{(2.97)} & 11.14 \scriptsize{(1.88)} & 23.14 \scriptsize{(3.52)} & 11.11 \scriptsize{(1.82)} \\
            % IO &  & \textit{20.28 \scriptsize{(2.61)}} & \textit{10.02 \scriptsize{(1.66)}} & \textbf{20.16 \scriptsize{(2.55)}} & \textbf{9.87 \scriptsize{(1.56)}} \\
            % IT & &  21.02 \scriptsize{(2.73)} & 10.46 \scriptsize{(1.74)} &  21.66 \scriptsize{(4.17)} & 10.20 \scriptsize{(1.78)} \\
            % OT & &  20.84 \scriptsize{(2.68)} & 10.27 \scriptsize{(1.70)} & 21.44 \scriptsize{(3.98)} & 10.02 \scriptsize{(1.68)} \\
            % IOT & & 20.46 \scriptsize{(2.68)} & 10.14 \scriptsize{(1.71)} & 21.28 \scriptsize{(3.97)} & 10.00 \scriptsize{(1.70)} \\
            
            \bottomrule
        \end{tabularx}
\end{table}

==> tables/results_baseline.tex <==
% (.*)\t(.*)\t0,(\d\d)(.*)\t0,(\d\d)(.*)\t0,(\d\d)(.*)
% \1 & \2 & \3.\4 & \5.\6 & \7.\8 \\\\

\newcolumntype{C}{>{\centering\arraybackslash}X}


\begin{table}
    \caption{Performances of the baseline models with mean (standard deviation), averaged on the target (T) population.}
    \label{table:res_baseline}
    % \begin{tabularx}{\linewidth}{C||C|C}
    %     \toprule
    %     \textbf{Model} & \textbf{RMSE} & \textbf{MAPE} \\ %& \textbf{TL} \\
    
         
    %      \midrule
         
    %      \textbf{FCN \#1} & 19.97 \scriptsize{(5.46)}  & 9.72 \scriptsize{(1.28)} \\
         
    %      \textbf{FCN \#2} & 18.56 \scriptsize{(4.75)} & 9.17 \scriptsize{(0.97)} \\ 
         
    %     \bottomrule
    % \end{tabularx}
    \begin{tabularx}{\linewidth}{c||C|C|C|C}
            \toprule
            
            \textbf{Dataset} & \multicolumn{2}{c|}{\textbf{FCN \#1}} & \multicolumn{2}{c}{\textbf{FCN \#2}} \\
            
            % \cmidrule{2-5}
            \midrule
            
             \textbf{T} & \textbf{RMSE} & \textbf{MAPE} & \textbf{RMSE} & \textbf{MAPE} \\
            
            \midrule
            
            ~I$^\dagger$ & 19.97 \scriptsize{(5.46)}  & 9.72 \scriptsize{(1.28)} & \textbf{18.56 \scriptsize{(4.75)}} & \textbf{9.17 \scriptsize{(0.97)}} \\
            O & 24.23 \scriptsize{(3.28)}  & 11.95 \scriptsize{(2.06)} & \textbf{22.31 \scriptsize{(2.94)}} & \textbf{11.15 \scriptsize{(1.90)}} \\
            
            
            \bottomrule
        \end{tabularx}
        
    \begin{flushright}
    \footnotesize{$^\dagger$ these results have first been presented in \cite{debois2019predictionatl}}
    \end{flushright}
\end{table}


==> tables/results_merged.tex <==

\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{Z}[1]{>{\centering}m{#1}}


\begin{table}
    \caption{Performances of the models after transfer for every Source (S) / Target (T) combination with mean (standard deviation), averaged on the target population.}
    \label{table:res_ft}
    \begin{tabularx}{\linewidth}{c|c||C|C|C|C}
            \toprule
            
            \multicolumn{2}{c||}{\textbf{Datasets}} & \multicolumn{2}{c|}{\textbf{FCN \#1}} & \multicolumn{2}{c}{\textbf{FCN \#2}} \\
            
            \midrule
            
            \textbf{S} & \textbf{T} & \textbf{RMSE} & \textbf{MAPE} & \textbf{RMSE} & \textbf{MAPE} \\
            
            \midrule
            
            - & I & 19.97 \scriptsize{(5.46)}  & 9.72 \scriptsize{(1.28)} & \textbf{18.56 \scriptsize{(4.75)}} & \textbf{9.17 \scriptsize{(0.97)}} \\
            - & O & 24.23 \scriptsize{(3.28)}  & 11.95 \scriptsize{(2.06)} & \textbf{22.31 \scriptsize{(2.94)}} & \textbf{11.15 \scriptsize{(1.90)}} \\
            
            \midrule
            \midrule
            
            \multicolumn{2}{c||}{\multirow{2}{*}{}} & \multicolumn{2}{c|}{\textbf{Standard Transfer}} & \multicolumn{2}{c}{\textbf{Adversarial Transfer}} \\
            
            \cmidrule{3-6}
            
             \multicolumn{2}{c||}{}  & \textbf{RMSE} & \textbf{MAPE} & \textbf{RMSE} & \textbf{MAPE} \\
            
            
            
            
            \midrule
            % \scriptsize{()} &  \scriptsize{()} &  \scriptsize{()} &  \scriptsize{()}
            
            I  & \multirow{7}{*}{I} & 16.46 \scriptsize{(4.24)} & 8.07 \scriptsize{(1.01)} & 15.42 \scriptsize{(3.97)} & 7.43 \scriptsize{(0.84)} \\
            O &  & 16.35 \scriptsize{(4.22)} & 8.02 \scriptsize{(1.00)} & 15.82 \scriptsize{(3.97)} &  7.74 \scriptsize{(0.90)} \\
            T &  & 17.97 \scriptsize{(4.74)} & 8.80 \scriptsize{(1.22)} & 17.88 \scriptsize{(4.85)} & 8.54 \scriptsize{(1.02)} \\
            IO &  & \textit{15.71 \scriptsize{(4.12)}} & \textit{7.70 \scriptsize{(0.97)}} & 15.30 \scriptsize{(3.78)} & 7.43 \scriptsize{(0.78)} \\
            IT &  & 16.24 \scriptsize{(4.23)} &  8.02 \scriptsize{(0.94)} & 15.39 \scriptsize{(4.05)} & 7.42 \scriptsize{(0.82)} \\
            OT &  & 16.21 \scriptsize{(4.18)} & 7.94 \scriptsize{(1.01)} & 15.64 \scriptsize{(4.09)} & 7.49 \scriptsize{(0.83)} \\
            IOT &  & 15.75 \scriptsize{(4.18)} & 7.75 \scriptsize{(1.00)} & \textbf{15.23 \scriptsize{(3.87)}} & \textbf{7.32 \scriptsize{(0.74)}} \\
            
            \midrule
            
            I  & \multirow{7}{*}{O} & 20.85 \scriptsize{(2.72)} & 10.34 \scriptsize{(1.79)} &  20.55 \scriptsize{(2.68)} & 10.08 \scriptsize{(1.71)} \\
            O & & 20.79 \scriptsize{(2.70)} & 10.22 \scriptsize{(1.70)} & 20.56 \scriptsize{(2.55)} & 10.08 \scriptsize{(1.60)} \\
            T &  & 22.65 \scriptsize{(2.97)} & 11.14 \scriptsize{(1.88)} & 23.14 \scriptsize{(3.52)} & 11.11 \scriptsize{(1.82)} \\
            IO &  & \textit{20.28 \scriptsize{(2.61)}} & \textit{10.02 \scriptsize{(1.66)}} & \textbf{20.16 \scriptsize{(2.55)}} & \textbf{9.87 \scriptsize{(1.56)}} \\
            IT & &  21.02 \scriptsize{(2.73)} & 10.46 \scriptsize{(1.74)} &  21.66 \scriptsize{(4.17)} & 10.20 \scriptsize{(1.78)} \\
            OT & &  20.84 \scriptsize{(2.68)} & 10.27 \scriptsize{(1.70)} & 21.44 \scriptsize{(3.98)} & 10.02 \scriptsize{(1.68)} \\
            IOT & & 20.46 \scriptsize{(2.68)} & 10.14 \scriptsize{(1.71)} & 21.28 \scriptsize{(3.97)} & 10.00 \scriptsize{(1.70)} \\
            
            \bottomrule
        \end{tabularx}
\end{table}

==> tables/results_tl_finetuned.tex <==

% \newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{Z}[1]{>{\centering}m{#1}}


\begin{table}
    \caption{Performances of the models after transfer for every Source (S) / Target (T) combination with mean (standard deviation), averaged on the target population.}
    \label{table:res_ft}
    \begin{tabularx}{\linewidth}{c|c||C|C|C|C}
            \toprule
            
            \multicolumn{2}{c||}{\textbf{Datasets}} & \multicolumn{2}{c|}{\textbf{Standard Transfer}} & \multicolumn{2}{c}{\textbf{Adversarial Transfer}} \\
            
            \midrule
            
            \textbf{S} & \textbf{T} & \textbf{RMSE} & \textbf{MAPE} & \textbf{RMSE} & \textbf{MAPE} \\
            
            \midrule
            % \scriptsize{()} &  \scriptsize{()} &  \scriptsize{()} &  \scriptsize{()}
            
            ~I$^\dagger$  & \multirow{7}{*}{I} & 16.46 \scriptsize{(4.24)} & 8.07 \scriptsize{(1.01)} & 15.42 \scriptsize{(3.97)} & 7.43 \scriptsize{(0.84)} \\
            O &  & 16.35 \scriptsize{(4.22)} & 8.02 \scriptsize{(1.00)} & 15.82 \scriptsize{(3.97)} &  7.74 \scriptsize{(0.90)} \\
            T &  & 17.97 \scriptsize{(4.74)} & 8.80 \scriptsize{(1.22)} & 17.88 \scriptsize{(4.85)} & 8.54 \scriptsize{(1.02)} \\
            IO &  & \textit{15.71 \scriptsize{(4.12)}} & \textit{7.70 \scriptsize{(0.97)}} & 15.30 \scriptsize{(3.78)} & 7.43 \scriptsize{(0.78)} \\
            IT &  & 16.24 \scriptsize{(4.23)} &  8.02 \scriptsize{(0.94)} & 15.39 \scriptsize{(4.05)} & 7.42 \scriptsize{(0.82)} \\
            OT &  & 16.21 \scriptsize{(4.18)} & 7.94 \scriptsize{(1.01)} & 15.64 \scriptsize{(4.09)} & 7.49 \scriptsize{(0.83)} \\
            IOT &  & 15.75 \scriptsize{(4.18)} & 7.75 \scriptsize{(1.00)} & \textbf{15.23 \scriptsize{(3.87)}} & \textbf{7.32 \scriptsize{(0.74)}} \\
            
            \midrule
            
            I  & \multirow{7}{*}{O} & 20.85 \scriptsize{(2.72)} & 10.34 \scriptsize{(1.79)} &  20.55 \scriptsize{(2.68)} & 10.08 \scriptsize{(1.71)} \\
            O & & 20.79 \scriptsize{(2.70)} & 10.22 \scriptsize{(1.70)} & 20.56 \scriptsize{(2.55)} & 10.08 \scriptsize{(1.60)} \\
            T &  & 22.65 \scriptsize{(2.97)} & 11.14 \scriptsize{(1.88)} & 23.14 \scriptsize{(3.52)} & 11.11 \scriptsize{(1.82)} \\
            IO &  & \textit{20.28 \scriptsize{(2.61)}} & \textit{10.02 \scriptsize{(1.66)}} & \textbf{20.16 \scriptsize{(2.55)}} & \textbf{9.87 \scriptsize{(1.56)}} \\
            IT & &  21.02 \scriptsize{(2.73)} & 10.46 \scriptsize{(1.74)} &  21.66 \scriptsize{(4.17)} & 10.20 \scriptsize{(1.78)} \\
            OT & &  20.84 \scriptsize{(2.68)} & 10.27 \scriptsize{(1.70)} & 21.44 \scriptsize{(3.98)} & 10.02 \scriptsize{(1.68)} \\
            IOT & & 20.46 \scriptsize{(2.68)} & 10.14 \scriptsize{(1.71)} & 21.28 \scriptsize{(3.97)} & 10.00 \scriptsize{(1.70)} \\
            
            \bottomrule
        \end{tabularx}
        
        \begin{flushright}
        \footnotesize{$^\dagger$ these results have first been presented in \cite{debois2019predictionatl}}
        \end{flushright}
\end{table}

==> tables/results_tl_global.tex <==

\newcolumntype{C}{>{\centering\arraybackslash}X}

\begin{table}
    \caption{Performances of the \textit{global} models after transfer for every Source (S) / Target (T) combination with mean (standard deviation), averaged on the population.}
    \label{table:res_global}
    \begin{tabularx}{\linewidth}{c|c||C|C|C|C}
        \toprule
        
        \multicolumn{2}{c||}{\textbf{Datasets}} & \multicolumn{2}{c|}{\textbf{Standard Transfer}} & \multicolumn{2}{c}{\textbf{Adversarial Transfer}} \\
        
        \midrule
        
        \textbf{S} & \textbf{T} & \textbf{RMSE} & \textbf{MAPE} & \textbf{RMSE} & \textbf{MAPE} \\
        
        \midrule
        
        % \scriptsize{()} &  \scriptsize{()} &  \scriptsize{()} &  \scriptsize{()}
        
        I  & \multirow{7}{*}{I} & 18.17 \scriptsize{(4.85)} & 8.67 \scriptsize{(0.78)} & 16.82 \scriptsize{(4.74)} & 8.14 \scriptsize{(0.95)} \\
        O & & 18.70 \scriptsize{(4.64)} & 9.22 \scriptsize{(0.86)} & 18.47 \scriptsize{(4.59)} & 8.97 \scriptsize{(0.80)} \\
        T &  & 33.49 \scriptsize{(6.65)} & 15.18 \scriptsize{(3.79)} & 44.53\scriptsize{(16.46)} & 19.80  \scriptsize{(5.34)} \\
        IO &  & \textit{17.07 \scriptsize{(4.81)}} & \textit{8.18 \scriptsize{(0.71)}} & \textbf{16.74 \scriptsize{(4.79)}} & 7.96  \scriptsize{(0.61)} \\
        IT &  & 18.90 \scriptsize{(5.72)} & 8.84 \scriptsize{(1.04)} & 18.01 \scriptsize{(6.42)} & 8.49 \scriptsize{(1.87)} \\
        OT &  & 20.14 \scriptsize{(4.50)} & 9.62 \scriptsize{(1.36)} & 18.44 \scriptsize{(4.43)} &  8.63 \scriptsize{(1.10)} \\
        IOT &  & 17.54 \scriptsize{(4.60)} & 8.25 \scriptsize{(0.65)} & 16.85 \scriptsize{(4.61)} & \textbf{7.79  \scriptsize{(0.65)}} \\
        
        \midrule
        
        I  & \multirow{7}{*}{O} & 22.54 \scriptsize{(2.33)} & 11.31 \scriptsize{(1.40)} & 22.84 \scriptsize{(1.72)} & 11.92 \scriptsize{(1.01)} \\
        O & & 21.20 \scriptsize{(2.45)} & 10.48 \scriptsize{(1.44)} & 20.99 \scriptsize{(2.36)} & 10.39 \scriptsize{(1.28)} \\
        T &  & 36.70 \scriptsize{(3.73)} & 19.05 \scriptsize{(4.45)} & 50.54\scriptsize{(10.18)} & 26.44  \scriptsize{(8.02)} \\
        IO &  & \textit{20.64 \scriptsize{(2.43)}} & 10.27 \scriptsize{(1.36)} & \textbf{20.49 \scriptsize{(2.37)}} & \textbf{10.16 \scriptsize{(1.23)}} \\
        IT & & 23.66 \scriptsize{(2.04)} & 12.45 \scriptsize{(1.34)} &  24.72 \scriptsize{(3.51)} & 13.27 \scriptsize{(2.08)} \\
        OT & & 21.23 \scriptsize{(2.56)} & 10.46 \scriptsize{(1.47)} & 21.28 \scriptsize{(2.61)} &  10.22 \scriptsize{(1.31)} \\
        IOT & & 20.67 \scriptsize{(2.50)} & \textit{10.26 \scriptsize{(1.50)}} & 20.76 \scriptsize{(2.53)} & 10.19 \scriptsize{(1.36)} \\
        
        \bottomrule
    \end{tabularx}
\end{table}
